Search for d^* Dibaryon by Double-radiative Capture on Pionic Deuterium

We report a search for d^* dibaryon production by double-radiative capture on pionic deuterium. The experiment was conducted at the TRIUMF cyclotron using the RMC cylindrical pair spectrometer, and detected gamma-ray coincidences following pion stops in liquid deuterium. We found no evidence for narrow dibaryons, and obtained a branching ratio upper limit, BR < 6.7 times 10^{-6} (90% C.L.), for narrow d^* production in the mass range from 1920 to 1980 MeV. Replaced with Physics Letter B accepted version and corrected normalization.

==> Makefile <==
# Makefile for xd tex
# $Id: Makefile,v 1.7 1999/11/03 04:28:43 zolnie Exp $
#
# $Log$
MAIN = ggnn
FIGS = detector.eps ggnn-fig?.eps  
SRCS = ggnn.tex $(FIGS) elsart*.sty elsart.cls 


all: 	
	-latex  $(MAIN) 
	-latex  $(MAIN)
	-latex  $(MAIN)
	-dvips  $(MAIN) -o $(MAIN).ps

$(MAIN).dvi: $(MAIN).tex
	-latex  $(MAIN) 	
	-latex  $(MAIN) 	


ps:  	$(MAIN).dvi
	-dvips -o $(MAIN).ps $(MAIN)

ps2:	ps
	psnup -Pletter -pletter -n 2  $(MAIN).ps > $(MAIN)-2up.ps

pdf:
	for i in $(FIGS); do echo "$$i -> PDF"; epstopdf $$i; done
	sed -e 's/\.eps/\.pdf/g' -e 's/dvips/pdftex/' -e 's/\%pdfver//g' < $(MAIN).tex > $(MAIN)-pdf.tex
	pdflatex $(MAIN)-pdf
	pdflatex $(MAIN)-pdf
	mv $(MAIN)-pdf.pdf $(MAIN).pdf

print:
	-lpr $(MAIN).ps

clean:
	-rm -f $(MAIN).ps $(MAIN)-2up.ps *.aux  *.dvi *.log *.blg *.out *.toc *.lof *.lot *~ $(MAIN).tgz

distclean:	clean

mrproper:	clean


tar:
	tar czvf $(MAIN).tgz $(MAIN).pdf $(SRCS) Makefile




